Semantic Evaluation for Text-to-SQL with Distilled Test Suites

We propose test suite accuracy to approximate semantic accuracy for Text-to-SQL models. Our method distills a small test suite of databases that achieves high code coverage for the gold query from a large number of randomly generated databases. At evaluation time, it computes the denotation accuracy of the predicted queries on the distilled test suite, hence calculating a tight upper-bound for semantic accuracy efficiently. We use our proposed method to evaluate 21 models submitted to the Spider leader board and manually verify that our method is always correct on 100 examples. In contrast, the current Spider metric leads to a 2.5% false negative rate on average and 8.1% in the worst case, indicating that test suite accuracy is needed. Our implementation, along with distilled test suites for eleven Text-to-SQL datasets, is publicly available.

==> other.tex <==
\section{Other Datasets}
We generated distilled test suites for \cosql{} \cite{yu-etal-2019-cosql}, \sparc{} \cite{yu-etal-2019-sparc}, Academic, Advising, ATIS, Geography, IMDB, Restaurants, Scholar and Yelp, where the later eight datasets are directly downloaded from \citet{finegan2018improving}.
Appendix \ref{sec:otherstats} include relevant statistics and examples of undistinguished neighbor queries.

We validate our approach on real model predictions for WikiSQL \cite{zhongSeq2SQL2017} in Appendix \ref{validateonwikisql}.
However, we recommend not to use test suite evaluation for this dataset, since there are no meaningful semantically equivalent queries.

